Large deviations in the quantum quasi-1D jellium

Wigner's jellium is a model for a gas of electrons. The model consists of $N$ unit negatively charged particles lying in a sea of neutralizing homogeneous positive charge spread out according to Lebesgue measure, and interactions are governed by the Coulomb potential. In this work we consider the quantum jellium on quasi-one-dimensional spaces with Maxwell-Boltzmann statistics. Using the Feynman-Kac representation, we replace particle locations with Brownian bridges. We then adapt the approach of Lebl\'e and Serfaty (2017) to prove a process-level large deviation principle for the empirical fields of the Brownian bridges.

==> defs.tex <==
% !TEX root = main.tex
\providecommand{\ms}{\mathsf}
\providecommand{\mb}{\mathbf}
\providecommand{\mc}{\mathcal}

% sets of numbers
\providecommand{\N}{\mathbb{N}}
\providecommand{\R}{\mathbb{R}}
\providecommand{\res}{\mathord{\upharpoonright}}
\providecommand{\Z}{\mathbb{Z}}
\providecommand{\T}{S}
\providecommand{\Tc}{S^{\ms{c}}}
\providecommand{\D}{D}
\providecommand{\Rd}{{\mathbb{R}^d}}
\providecommand{\K}{\T}
\newcommand{\Zd}{{\mathbb{Z}^d}}
\providecommand{\Q}{\mathbb{Q}}
\providecommand{\W}{\mathbb{W}}
\providecommand{\G}{\Gamma}

% probability measures 
\renewcommand{\P}{\mathbb{P}}
\providecommand{\Pc}{\P^{\ms C}}
\providecommand{\Pca}{\P^{\ms C, 1}}
\providecommand{\Pcb}{\P^{\ms C, 2}}
\providecommand{\Fc}{F^{\ms C }}
\providecommand{\Ec}{\E^{\ms C}}
\providecommand{\oP}{\overline{\mathbb{P}}}
\providecommand{\oE}{\overline{\mathbb{E}}}
\providecommand{\E}{\mathbb{E}}
\providecommand{\Ee}{E_\eta}
\providecommand{\Cc}{\mc{C}}
\providecommand{\Cco}{\mc C^{\ms C}}
\providecommand{\C}{\mathfrak{C}}
\providecommand{\Lip}{\ms{Lip}}
\providecommand{\scr}{\ms{scr}}
\providecommand{\Cr}{\CC^{\ms{reg}}}
\providecommand{\Cs}{\CC^{\scr}}
\providecommand{\Css}{\CC^*}
\providecommand{\Cm}{\CC^{\ms{good}}}
\renewcommand{\H}{\mc{H}}
\providecommand{\tH}{\tilde\mc{H}}
% aux
\providecommand{\wt}{\widetilde}
\renewcommand{\d}{{\rm d}}
\providecommand{\PBB}{\P_{\ms{BB},N}}
\providecommand{\dd}{{\rm d}}
\providecommand{\mun}{\mu_{N, \b}}
\providecommand{\dist}{\ms{dist}}
\providecommand{\disc}{\Delta}
\providecommand{\ran}{\ms{ran}}
\providecommand{\es}{\emptyset}
\providecommand{\one}{\mathbbmss{1}}
\providecommand{\eps}{\varepsilon}
\providecommand{\calC}{\mc{C}}
\providecommand{\calD}{\mc{D}}
\providecommand{\per}{\ms{per}}
\providecommand{\Ps}{\mc{P}_{\ms{s}}}
\providecommand{\Pu}{\mc{P}}
\providecommand{\Ii}{I^{(i)}}
\providecommand{\Pl}{\hspace{-.2cm}P}
\providecommand{\Phm}{\Phi^{\ms{good}}_{\de, U,  N}}
\providecommand{\Phs}{\Phi^{\scr}_{\delta, R}}
\providecommand{\Es}{E^{\scr}}
\providecommand{\Eo}{E^{(R, \e)-\ms{opt}}}
\providecommand{\ER}{\mc{E}_{R}}
%\providecommand{\ERt}{\mc{E}_{R,t}}
\providecommand{\ENt}{\mc{E}_{N,t}}
\providecommand{\Pst}{\mc{P}_s}
\providecommand{\ent}{{\ms{ent}}}
\providecommand{\Elec}{\ms{Elec}^*}
\providecommand{\Elecs}{\ms{Elec}}
\providecommand{\Ent}{\ent}
\providecommand{\Pois}{\ms{Pois}}
\providecommand{\Bin}{\ms{Bin}}
\providecommand{\Conf}{\ms{Conf}}
\providecommand{\ConfbN}{\ms{Conf}_{\beta, N}}
\providecommand{\ConfN}{\ms{Conf}_{N}}
\providecommand{\ConfbR}{\ms{Conf}_{\beta, R}}
\providecommand{\ConfR}{\ms{Conf}_R}
\renewcommand{\o}{\overline}
\renewcommand{\div}{\ms{div}\,}

%bar notation
\providecommand{\Emp}{\ms{Emp}_N}
\providecommand{\Comp}{\ms{Comp}}
\providecommand{\CA}{\ms{ContAv}}
\providecommand{\DA}{\ms{Avg}_R}
\providecommand{\Sc}{\ms{Scr}}
\providecommand{\Scr}{\ms{Scr}}
\providecommand{\Fm}{F^{M}_{R,\eta}}
\providecommand{\Om}{\mc{O}^{M, }_{R,\eta}}
\providecommand{\Sm}{\mc{S}^{M, }_{R,\eta}}
\renewcommand{\mod}{\ms{mod}}
%\providecommand{\reg}{\ms{reg}}
\providecommand{\vXN}{\vec{X}_N}
\providecommand{\vGN}{{\Gamma}_N}
\providecommand{\vgN}{\CC}%{\vec{\gamma}_N}
\providecommand{\gN}{g}
\providecommand{\vzN}{\vec{z}_N}
\providecommand{\fPN}{{\mathfrak{P}}_{N,\beta}}
\providecommand{\fQN}{\overline{\frak{Q}}_{N,\beta}}
\providecommand{\Fmod}{F^{\ms{mod}}}
\providecommand{\WR}{\frac1R W_{S_R}}
\providecommand{\WRM}{\W^{R, M}}
\providecommand{\WRR}{\W^{R}}
\providecommand{\WM}{\mc W^{\wedge M}}
\providecommand{\NR}{\mc N_R(P)}
\providecommand{\NdR}{\mc N_{\delta, R}(P)}
\providecommand{\Nd}{\mc N_\delta(P)}
\providecommand{\FMRe}{M \wedge \WR}
\providecommand{\rpp}{x_-}
\providecommand{\rmm}{x_+}
\providecommand{\cm}{c_{\ms{mov}}}

% greeks
\renewcommand{\t}{\tau}
\providecommand{\s}{\sigma}
\providecommand{\g}{\gamma}
\providecommand{\e}{\varepsilon}
\renewcommand{\b}{\beta}
\providecommand{\la}{\lambda}
\providecommand{\de}{\delta}

%

%color
\newcommand{\blue}[1]{{\textcolor{blue}{{\bf \emph{#1}}}}{}}
\newcommand{\red}[1]{{\textcolor{red}{{\bf \emph{#1}}}}{}}
\def\tcb{\textcolor{blue}}
\def\tcr{\textcolor{red}}
\def\tcg{\textcolor{green}}
\def\tcm{\textcolor{magenta}}

%Paul defs
\def\fdd{\stackrel{fdd}{\Longrightarrow}}
\def\ed{\stackrel{d}{=}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\aa{\alpha}
\def\bb{\beta}
\def\bbE{\mathbb{E}}
\def\bbP{\mathbb{P}}
\def\eps{\epsilon}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\nn{\nonumber}
\def\ff{\infty}
\def\({\left(}
\def\){\right)}
\def\[{\left[}
\def\]{\right]}
\def\lk{\left\{}
\def\rk{\right\}}
\def\lb{\left|}
\def\rb{\right|}
\def\lc{\lceil}
\def\rc{\rceil}
\def\lf{\lfloor}
\def\rf{\rfloor}
\def\Cov{\text{Cov}}
\def\Var{\text{Var}}
\def\sign{\text{sign}}

\def \P{\mathbb{P}}
\def \E{\mathbb{E}}
\def \V{\mathbf{V}}
\def \AA{{\cal A}}
\def \BB{{\cal B}}
\def \CC{{\mc C}}
\def \CCBB{{\CC}}
\def \CP{\CC^{\ms{Pois}}}
\def \CCBBB{{\CC'}}
\def \DD{{\cal D}}
\def \EE{{\cal E}}
\def \FF{{\cal F}}
\def \GG{{\cal G}}
\def \HH{{\cal H}}
\def \II{{\cal I}}
\def \JJ{{\cal J}}
\def \KK{{\cal K}}
\def \LL{{\mc L}}
\def \MM{{\cal M}}
\def \NN{{\cal N}}
\def \OO{{\cal O}}
\def \PP{{\cal P}}
\def \QQ{{\cal Q}}
\def \RR{{\cal R}}
\def \SS{{\cal S}}
\def \TT{AAAA}
\def \TTc{I^{\ms{c}}}
\def \UU{{\cal U}}
\def \VV{{\cal V}}
\def \WW{{\cal W}}
\def \XX{{\cal X}}
\def \YY{{\cal Y}}
\def \ZZ{{\cal Z}}

\def\been{\begin{enumerate}}
\def\enen{\end{enumerate}}
\def\im{\item}

